Globally optimal registration of noisy point clouds

Registration of 3D point clouds is a fundamental task in several applications of robotics and computer vision. While registration methods such as iterative closest point and variants are very popular, they are only locally optimal. There has been some recent work on globally optimal registration, but they perform poorly in the presence of noise in the measurements. In this work we develop a mixed integer programming-based approach for globally optimal registration that explicitly considers uncertainty in its optimization, and hence produces more accurate estimates. Furthermore, from a practical implementation perspective we develop a multi-step optimization that combines fast local methods with our accurate global formulation. Through extensive simulation and real world experiments we demonstrate improved performance over state-of-the-art methods for various level of noise and outliers in the data as well as for partial geometric overlap.

==> modeling.tex <==
\section{Problem Formulation}
\label{sc:modeling}
\input{notation}
Let us consider the problem of registering a set of points in the sensor frame $\mS=\{\bss_1,\dots,\bss_{n_{\mS}}\}$ ($\bss_i\in\Real^3$) to a model of an object given by vertices $\mV=\{\bv_1,\dots, \bv_{n_{\mV}}\}$ ($\bv_i,\bss_i\in\Real^3$) and $n_{f}$ faces. Let $\bF\in{0,1}^{n_{\mV}\times n_f}$ be the binary map that captures the vertices forming each face. Let $\bC\in\Real^{n_{\mS}\times n_{\mV}}$ be a matrix that assigns the point correspondence and $\bff\in\{0,1\}^{n_{\mS}\times n_f}$ be the matrix that assigns face correspondence. Let $\bSigma_{\bss_i}$ be the covariance associated with the sensor points, such that $\bss_i \sim \mN(\widehat{\bss_i},\bSigma_{\bss_i})$. We assume that each sensor point $\bss_i$ corresponds to a unique point on the model. We follow the maximum likelihood estimate (MLE) approach of Segal~\etal~\cite{} to pose point cloud registration as an optimization problem shown below,
\begin{align}
\label{eq:eq0}
&\min_{\bR,\bt,\bC,\bff} && O(\bR,\bt,\bC,\bff)\\ 
\label{eq:eq1}
&\text{where} \quad && O =\frac{1}{n_{\mS}}\sum_{i=1}^{n_{\mS}}\bd_i^T (\bR \bSigma_{\bss_i} \bR^T)^{-1} \bd_i, \\
& &&\bd_i= \bR\bss_i+\bt-\mV{\bC_i}^{T},\nonumber\\
\label{eq:RSO3}
&\text{subject to}  \quad && \bR^T\bR=\bI_{3\times 3}, \det(\bR)=1  \\
& &&\sum_{j=1}^{n_{\mV}}\bC_{i,j}=1, \quad \forall i,\nonumber\\
& &&\sum_{k=1}^{n_{f}}\bff_{i,k}=1, \quad \forall i,\nonumber\\
& &&0\leq \bC_{i,j} \leq \bF_j \bff_i^T, \quad \forall i,j,\nonumber\\
& &&\bff_{i,j}\in \{0,1\}, \quad \forall i,j,\nonumber
\end{align}
where $\bR\in\SO$ is the rotation matrix and $\bt\in\Real^3$ is the translation vector and the notation $\bA_i$ refers to the $i^{\text{th}}$ row of $\bA$. 
Simplifying Eq.~\ref{eq:eq1}, we get 
\begin{align}
O &=\frac{1}{n_{\mS}}\sum_{i=1}^{n_{\mS}} (\bR^T \bd_i)^T\bSigma_{\bss_i}^{-1} (\bR^T \bd_i) \nonumber\\
&=\frac{1}{n_{\mS}}\sum_{i=1}^{n_{\mS}}\be_i^T\bSigma_{\bss_i} ^{-1}\be_i,\nonumber\\
\text{where} \quad &\be_i=\bss_i-\bt'-\bR'\mV\bC_i^T,\nonumber \\
\label{eq:R't'}
&\bt'=-\bR^T\bt, \bR'=\bR^T. \\
\Rightarrow O&=\frac{1}{n_{\mS}}\sum_{i=1}^{n_{\mS}}||\bB_i^T (\bR'\mV\bC_i^T+\bt'-\bss_i)||^2_2,
\end{align}
where $\bB_i\in\Real^{3\times 3}$ is obtained from a Cholesky decomposition of $\bSigma_{\bss_i}$ (\emph{i.e.} $\bB_i\bB_i^T=\bSigma_{\bss_i}$). Further, it is worth noting that we have transformed the problem of estimating $\bR,\bt$ that transform sensor points to the model, to an alternate version that transforms model to the sensor points. Once we estimate $\bR',\bt'$, we can obtain $\bR, \bt$ from Eq.~\ref{eq:R't'}.

  
In order to keep the problem quadratic in terms of the optimization variables, we switch to an L-1 norm (One could also switch to an L-$\infty$ norm as shown by Yu~\etal~\cite{}),
\begin{align}
O &=\frac{1}{n_{\mS}}\sum_{i=1}^{n_{\mS}}|\bB_i^T (\bR'\mV\bC_i^T+\bt'-\bss_i)|.
\end{align}
Note that, if one were to substitute $\bSigma_{\bss_i}=\bI_{3\times 3}$ in Eq.~\ref{eq:eq1}, the objective function would trivially simplify to the form used by Izatt~\etal~\cite{}. 

The optimization problem stated above is already a mixed integer quadratic programming problem except for the constraints associated with $\bR'$ in Eq.~\ref{eq:RSO3}. We follow the approach of Dai~\etal to approximate the constraint on $\bR'$. If we assume 
$\bR' =\begin{bmatrix}
\br_1 & \br_2 & \br_3
\end{bmatrix}$, then the approximate constraints are
\begin{subequations}
	\label{eq:Rconstraints}
\begin{align}
&\begin{bmatrix}
\br_{i,j}\\
\bw_{i,j}
\end{bmatrix}=\sum_{k=0}^{n}\lambda_k^{i,j}\begin{bmatrix}
\frac{2 k-n}{n}\\ 
\left(\frac{2 k-n}{n}\right)^2
\end{bmatrix}, \quad \bw \in \Real^3, \ j=1,2,3,  \\
\label{eq:sos21}
&\text{where} \quad \sum_{k=0}^{n} \lambda_k =1, \lambda_k \geq 0, \\
\label{eq:sos22}
&\exists j \in 0,\dots,n-1,	\lambda_k=0 \forall k \neq j,k\neq j+1,\\
&\br_i^T\br_i\leq 0, \\
&\mathbbm{1}^T\bw_{i}\geq 1,\\
& (\br_i\pm \br_j)^T(\br_i\pm \br_j)\leq 2,\\
& (\br_1\pm \br_2 \pm \br_3)^T(\br_1\pm \br_2 \pm \br_3)\leq 3.
\end{align}
\end{subequations}
Constraints Eq.~\ref{eq:sos21},~\ref{eq:sos22} are referred to as special ordered set of type 2 (sos2) constraint in the MIP literature~\cite{beale1970special}. 
An observation we make is that when performing MIP, reducing the number of discreet variables greatly reduces the computation time when compared to continuous variables. As a result, instead of using $\bf$ to find the closest face and then the closest point on that face using $\bC$, we adopt a faster albeit approximate approach. We generate several points on each face $\mM=\{\bm_1,\dots, \bm_{n_{\mM}}\}$ ($\bm_i\in\Real^3$) and use a correspondence matrix $\bC^b\in\{0,1\}^{n_{\mS}\times n_{\mM}}$ to find the correspondence from each sensor point to one of the generated model points. 
We thus rewrite the optimization problem as shown below,
\begin{align}
\label{eq:GMIP}
&\min_{\bR',\bt',\bC^b,\bphi,\balpha,\bo} &&\frac{1}{n_{\mS}}\sum_{i=1}^{n_{\mS}}\phi_i,\\
&\text{subject to} \quad &&\phi_i \geq \mathbbm{1}^T \balpha_i,\nonumber\\
& && \phi_i \geq \phi_{max} o_i,\nonumber\\
& && \balpha_i \geq +\bB_i^T (\bR'\mM(\bC^b_i)^T+\bt'-\bss_i)-\gamma o_i,\nonumber\\
& && \balpha_i \geq -\bB_i^T (\bR'\mM(\bC^b_i)^T+\bt'-\bss_i)-\gamma o_i,\nonumber\\
& && \sum_{i=1}^{n_{\mM}} \bC^b_{i,j}+o_i=1,\nonumber\\
& &&\phi_i,\alpha_{i,j}\geq 0,\nonumber\\
& && o\in \{0,1,\}^{n_{\mS}},\bC^b \in \{0,1\}^{n_{\mS} \times n_{\mM}},\nonumber\\
& && \text{Constraints on $\bR'$ from Eq.~\ref{eq:Rconstraints}}\nonumber
\end{align}
where $\phi_{max}$ and $\gamma$ are threshold values used for classifying points as outliers.




